Improving Viewpoint Consistency in 3D Generation via Structure Feature and CLIP Guidance

Despite recent advances in text-to-3D generation techniques, current methods often suffer from geometric inconsistencies, commonly referred to as the Janus Problem. This paper identifies the root cause of the Janus Problem: viewpoint generation bias in diffusion models, which creates a significant gap between the actual generated viewpoint and the expected one required for optimizing the 3D model. To address this issue, we propose a tuning-free approach called the Attention and CLIP Guidance (ACG) mechanism. ACG enhances desired viewpoints by adaptively controlling cross-attention maps, employs CLIP-based view-text similarities to filter out erroneous viewpoints, and uses a coarse-to-fine optimization strategy with staged prompts to progressively refine 3D generation. Extensive experiments demonstrate that our method significantly reduces the Janus Problem without compromising generation speed, establishing ACG as an efficient, plug-and-play component for existing text-to-3D frameworks.

==> method_12-11.tex <==
\section{Method}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/attention_map.png}
    \caption{\textbf{Average attention maps.} As the prompt complexity increases, the diffusion model's attention to viewpoint token decreases significantly.}
    \label{fig:attention_map}
\end{figure}

\subsection{Rethink Janus Problem}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/Pipeline.png}
    \caption{\textbf{Overview of our work.} We adjusts cross-attention maps in the diffusion model to enhance focus on orientation keywords, guiding the model to generate diverse viewpoints. CLIP supervision prunes incorrect orientations during denoising based on a loss threshold, ensuring alignment with specified viewpoints. Decompose the original prompt into object and descriptive words, and optimizing the object prompt in the early stages to ensure geometric integrity.}
    \label{fig:pipeline}
\end{figure*}


\textbf{Change of Data Distribution Over Time.} The diffusion process can be described using both the forward and reverse SDEs. By applying the Fokker-Planck equation to forward SDE~\cite{song2020score}, we can derive:
\[
\scriptsize
\frac{\partial p_t(x)}{\partial t} = - \nabla_x \cdot \left( \left( f(x,t) - \frac{1}{2} g^2(t) \nabla_x \log p_t(x) \right) p_t(x) \right), \tag{5}
\]

This represents the change of the original data distribution \( p(x) \) over time \( t \) from \( 0 \) to \( T \), eventually converging to a standard Gaussian distribution.

For the reverse SDE, let \( s = T - t \), we can obtain a forward process from \( s = 0 \) to \(  T \). The Fokker-Planck equation for the reverse SDE can be written as:

\[
\scriptsize
\frac{\partial q_s(x)}{\partial s} = - \nabla_x \left[ \left( \frac{1}{2} g^2(t) \cdot \nabla_x \log p_t(x) - f(x,t) \right) \cdot q_s(x) \right], \tag{6}
\]

This represents the change of the Gaussian distribution over time \( s \) from 0 to \( T \) (which corresponds to \( t \) from \( T \) to 0), and it is the reverse of equation (5). Therefore, when the predicted noise during the reverse process is accurate enough, the generated data will recover the distribution of the training data.

\noindent \textbf{Revisiting SDS.} The SDS formula proposed by DreamFusion~\cite{poole2022dreamfusion} can be expressed as:

\[
\scriptsize
\nabla_{\theta} \mathcal{L}_{\text{SDS}}(\theta) \approx \mathbb{E}_{t,\epsilon,c} \left[ \omega(t) \left( \epsilon_{\phi}(x_t, t, y) - \epsilon \right) \frac{\partial g(\theta, c)}{\partial \theta} \right], \tag{7}
\]

where \(\epsilon\) represents the 2D rendered image \( x_0 = g(\theta, c) \) of a 3D object, with standard Gaussian noise added at time \( t \). The symbol \( \epsilon_{\phi} \) represents the noise predicted by the UNet for the given prompt and noisy image.

Let \( \gamma(t) = \frac{\sqrt{1 - \bar{\alpha}_t}}{\sqrt{\bar{\alpha}_t}} \), and from DDPM~\cite{ho2020denoising}, \( \bar{x}_0^t = \frac{x_t - \sqrt{1 - \bar{\alpha}_t} \epsilon_{\phi}(x_t, t, y)}{\sqrt{\bar{\alpha}_t}} \), Eq.(7) can be transformed in to:

\[
\nabla_{\theta} \mathcal{L}_{\text{SDS}}(\theta) = \mathbb{E}_{t,\epsilon,c} \left[ \frac{\omega(t)}{\gamma(t)} \left( x_0 - \bar{x}_0^t \right) \frac{\partial g(\theta, c)}{\partial \theta} \right]. \tag{8}
\]

In this sense, we can regard SDS as guiding the rendered 3D images using the generated images from Diffusion~\cite{liang2024luciddreamer}. The long-tailed distribution of viewpoints in the training data—where most images are front-facing—introduces bias in the generated images show as Figure(\ref{fig:long_tail}). When the distribution of the generated images exhibits a long-tailed distribution, the guidance becomes imbalanced, leading to overfitting of the 3D object to images from the highest density region. 

Second, when the Janus problem is attributed to guidance in 2D diffusion image generation, we find that the generated object is influenced not only by the distribution of the training data but also by the improper guidance from the input prompt. Specifically, popular text-to-3D models currently modify the original input text based on the rendering angle \( v \) of the current 3D representation, producing phrases like “prompt, * view,” where * often corresponds to front, side, or back. This approach aims to optimize the 3D representation by providing directional textual guidance. In Figure(\ref{fig:attention_map}), we demonstrate that as prompt complexity increases, the model’s focus on directional terms decreases significantly. Inspired by these two observations, we aim to address the aforementioned issues to achieve improved outcomes.

\subsection{Cross Attention Control}
The Janus Problem arises from viewpoint bias in generative models, resulting in the production of pseudo-ground truth \( \tilde{x_0} \), which misguides the rendered image \( x_0 = g(\theta, c) \).

Our approach directs the model to generate images from low-probability density regions without altering the training data or fine-tuning the model.

\noindent \textbf{Cross-attention in U-Net.} This study employs Stable Diffusion as the base model. In the architecture of Stable Diffusion, cross-attention layers are embedded within the encoding and decoding stages of the U-Net, merging text and image features by mapping spatial features of \( z_t \), \( \phi(z_t) \), to a query matrix \( Q = l_Q(\phi(z_t)) \). The text embedding \( \psi(P) \) is mapped to key and value matrices, \( K = l_K(\psi(P)) \) and \( V = l_V(\psi(P)) \). The attention map
\[
M = \text{Softmax} \left( \frac{QK^T}{\sqrt{d}} \right),\tag{9}
\]
weights \( V \) to produce \( MV \), which updates \( \phi(z_t) \).

This cross-attention aligns each noise prediction step with the text prompt, while self-attention layers handle interactions among image features only. Our method mainly adjusts the text prompt’s embedding channels in cross attention.

\noindent
\textbf{Cross Attention Control.} Our method improves the probability of the diffusion model generating images with the correct viewpoint by adjusting the cross-attention map \( M \). The cross-attention map \( M \) is determined by both the latent variables and text prompts (as shown in Equation 9) and is based on the similarity between the query vector \( Q \) and the key vector \( K \), with dimensions matching the length of the tokens in the text prompt.

At each noise prediction step in the U-Net during the diffusion process, we locate orientation-related keywords in the cross-attention map. Then, based on the desired rendering perspective, we dynamically adjust the attention weights of these orientation keywords. This adjustment is achieved with the following formula:
\[
M' = M \times (1 + \lambda \cdot \mathbf{I}_{\text{keywords}}), \tag{10}
\]

where, \( M \in \mathbb{R}^{N \times T} \) is the original cross-attention map, with \( N \) representing the dimension of latent variables and \( T \) the number of tokens in the text prompt. \( \lambda \) is an adjustment coefficient that controls the enhancement or reduction of attention; positive values increase attention, while negative values decrease it. \( \mathbf{I}_{\text{keywords}} \in \mathbb{R}^{N \times T} \) is an indicator matrix where elements corresponding to orientation keywords are set to 1, and others are set to 0.
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/example3.png}
    \caption{\textbf{Comparison with baselines methods in text-to-3D generation.} Adding our method to the baseline significantly improves geometric consistency without increasing optimization time or compromising generation quality.}
    \label{fig:example}
\end{figure*}

By selectively amplifying or reducing the model's attention to orientation keywords, we guide the model to focus more on relevant orientation information, thereby increasing the probability of generating images with the correct viewpoint.

\subsection{Coarse-to-Fine Optimization and CLIP Pruning}
\noindent
\textbf{Coarse-to-fine optimization Based on Prompt.} In this study, we observed a notable reduction in the diffusion model’s ability to maintain attention on individual words as prompt complexity increased. To address this issue, we propose a two-stage optimization approach for 3D generation, designed to enhance the model’s focus on essential elements within complex prompts.

First, using GPT4o, we segment the input prompt into two parts: the object prompt representing the main subject, and the description prompt which provides additional characteristics of the object. In the initial stage, our approach focuses on object prompt by controlling cross attention and CLIP pruning to selectively increase focus on the primary subject. This step helps ensure that the generated 3D model accurately captures the core theme of the prompt. In the subsequent stage, we introduce the description prompt to add detailed visual characteristics, thereby improving the model’s ability to capture finer aspects and increasing the realism of the 3D output.

\noindent
\textbf{CLIP Pruning.} During the optimization, we also proposed a pruning strategy to ensure that the guidance from the diffusion model aligns with the current rendering view, effectively addressing the Janus problem. In each training iteration, we extract a "pseudo ground truth" image \( \hat{\mathbf{x}}_0 \) from the denoised latents. We then compute the CLIP loss between \( \hat{\mathbf{x}}_0 \) and a text prompt \( P_\theta \), where \( \theta \) is the azimuth angle corresponding to the rendering view. If the CLIP loss is below a set threshold, the iteration is skipped.

The pruning threshold \( \tau \) is determined using CLIP loss statistics collected during the initial epoch, where no pruning is applied. Specifically, \( \tau \) is defined as:
\[
\tau = \alpha \cdot \lambda_{\min} + (1 - \alpha) \cdot \lambda_{\text{mean}}, \tag{11}
\]
where \( \lambda_{\min} \) and \( \lambda_{\text{mean}} \) represent the minimum and mean CLIP loss values, respectively, and \( \alpha \in [0, 1] \) is a tunable hyperparameter controlling the pruning sensitivity.

This approach effectively filters out erroneous view-dependent guidance provided by the diffusion model, enabling more accurate optimization of NeRF and thereby addressing the Janus problem effectively.

==> sec/supp_sec.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary



\section{Formula Derivation }
\label{sec:formula}

Assume that the initial data distribution \( p_{\text{data}}(x) \) follows a long-tailed distribution. We aim to prove that \( q_{\text{generation}}(x) \) also follows a long-tailed distribution.


\subsection{Forward process}
We know the SDE of the forward Diffusion process was given by~\cite{song2020score}:

\begin{equation}
dx = f(x, t)dt + g(t)dW \tag{1}
\end{equation}

From this, we derive the Fokker-Planck equation~\cite{oksendal2013stochastic, risken1996fokker} which governs the time evolution of the probability density function \( p_t(x) \):

\begin{equation}
\frac{\partial p_t(x)}{\partial t} = -\nabla_x \cdot \left( f(x, t) p_t(x) \right) + \frac{1}{2} g(t)^2 \nabla_x^2 p_t(x) \tag{2}
\end{equation}

Next, we present the gradient formula linking the log-density gradient to the density gradient:

\begin{equation}
\nabla_x \log p_t(x) = \frac{\nabla_x p_t(x)}{p_t(x)}
\tag{3}
\label{equation3}
\end{equation}

Substituting this into the diffusion term gives:

\[
\frac{1}{2} g(t)^2 \nabla_x^2 p_t(x) = \frac{1}{2} g(t)^2 \nabla_x \cdot \left( p_t(x) \nabla_x \log p_t(x) \right)
\]

Finally, we combine the diffusion and drift terms by substituting the above result into the Fokker-Planck equation:

\[
\frac{\partial p_t(x)}{\partial t} = \begin{aligned}[t]
&- \nabla_x \cdot \left( f(x, t) p_t(x) \right) \\
&+ \nabla_x \cdot \left( \dfrac{1}{2} g(t)^2 p_t(x) \nabla_x \log p_t(x) \right)
\end{aligned}
\]
By merging the two divergence terms, we arrive at the final form of the Fokker-Planck equation:

\begin{equation}
\frac{\partial p_t(x)}{\partial t} = -\nabla_x \cdot \left[ \left( f(x, t) - \frac{1}{2} g(t)^2 \nabla_x \log p_t(x) \right) p_t(x) \right] \tag{4}
\label{equation4}
\end{equation}



\subsection{Reverse process}

We know the SDE of the reverse Diffusion process was given by~\cite{song2020score}:

\begin{equation}
dx = \left[f(x, t) - g(t)^2 \nabla_x \log p_t(x)\right] dt + g(t) d\Bar{w} \tag{5}
\end{equation}

Assuming the initial \( q_T(x) \sim \mathcal{N}(0, 1) \), we aim to determine how \( q_t(x) \) evolves over the time interval \( t \in [T, 0] \).

To facilitate this, we introduce a new time variable \( s = T - t \), where \( s \) increases from \( 0 \) to \( T \) as \( t \) decreases from \( T \) to \( 0 \). Consequently, the differential relationship becomes:

\[
ds = -dt
\]

Rewriting the reverse SDE in terms of the new time variable \( s \), we obtain:

\begin{equation}
dx = \left[-f(x, t) + g(t)^2 \nabla_x \log p_t(x)\right] ds + g(t) d{w} \tag{6}
\end{equation}

Here, \( d{w} \) represents a forward Wiener process in the new time \( s \).
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/sup_1.png}
    \caption{As the cross attention control ratio for token “back” increases, the front features gradually disappear and the back features emerge.}
    \label{fig:sup_1}
\end{figure*}
Using the Fokker-Planck equation, the evolution of \( q_s(x) \) with respect to time \( s \) is described by:

\begin{equation}
\begin{aligned}
\frac{\partial q_s(x)}{\partial s} ={} & -\nabla_x \cdot \left\{ q_s(x) \left[ -f(x, t) + g(t)^2 \nabla_x \log p_t(x) \right] \right\} \\
&\quad + \frac{1}{2} g(t)^2 \nabla_x^2 q_s(x)
\end{aligned}
\tag{7}
\end{equation}


Using Eq.~\ref{equation3}, we have:

\begin{equation}
\begin{aligned}
\frac{\partial q_s(x)}{\partial s} = 
\nabla_x \cdot \Big[ \Big( & f(x, t) 
- g(t)^2 \nabla_x \log p_t(x) \\
& + \frac{1}{2} g(t)^2 \nabla_x \log q_s(x) \Big) q_s(x) \Big]
\end{aligned}
\tag{8}
\end{equation}



The forward time step \( t \) and the reverse time step \( s \) represent the same point in time.
The key to the reverse process, inverting the forward process, lies in accurately estimating the score function \( \nabla_x \log p_{t}(x) \). In practice, this estimation is performed by training a neural network to approximate the true score function. If the neural network provides an accurate estimate:

\[
\begin{aligned}
\nabla_x \log q_s(x) \approx \nabla_x \log p_t(x)
\end{aligned}
\]


Finally, rearranging the terms leads to:

\begin{equation}
\frac{\partial q_s(x)}{\partial s} = -\nabla_x \cdot \left[ \left( \frac{1}{2} g(t)^2 \nabla_x \log p_t(x) - f(x, t) \right) q_s(x) \right] \tag{9}
\label{equation9}
\end{equation}

\subsection{Evolution of Data Distribution Over Time}
From the perspective of \textbf{probability flow density}, the Fokker-Planck equation describes how the probability density function (PDF) evolves over time under stochastic dynamics. In our derivation, we obtained the Fokker-Planck equation for the forward SDE as shown in equation (4):

\[
\frac{\partial p_t(x)}{\partial t} = -\nabla_x \cdot \left[ \left( f(x, t) - \frac{1}{2} g(t)^2 \nabla_x \log p_t(x) \right) p_t(x) \right]
\]

This equation characterizes the time evolution of the probability density \( p_t(x) \) influenced by the drift term \( f(x, t) \) and the diffusion term involving the gradient of the log-density \( \nabla_x \log p_t(x) \).

In the reverse process, we introduce a new time variable \( s = T - t \) to effectively reverse the time direction. The Fokker-Planck equation for the reverse SDE, derived in equation (9), is given by:

\[
\frac{\partial q_s(x)}{\partial s} = -\nabla_x \cdot \left[ \left( \frac{1}{2} g(t)^2 \nabla_x \log p_t(x) - f(x, t) \right) q_s(x) \right]
\]

Here, the drift and diffusion terms have signs opposite to those in the forward equation, and the time derivative is with respect to \( s \), reflecting the reversal of time. 

From the probability flow density viewpoint, this sign reversal implies that the reverse Fokker-Planck equation effectively inverts the probability flow dictated by the forward equation. The probability density \( q_s(x) \) in the reverse process evolves in a manner that retraces the evolution of \( p_t(x) \) in the forward process but in reverse time. This ensures that the reverse SDE undoes the effect of the forward SDE on the probability density, allowing the generative distribution \( q_{\text{generation}}(x) \) to approximate the original data distribution \( p_{\text{data}}(x) \).

Therefore, based on our derivations leading to equations~\ref{equation4} and~\ref{equation9}, we can conclude that the Fokker-Planck equation for the reverse SDE is indeed the reverse process of the forward SDE's Fokker-Planck equation. This explains how the reverse diffusion process successfully reconstructs samples from the data distribution by inverting the probability flow of the forward process. This also reveals that the long-tail distribution of the training data of the diffusion model affects the distribution of the generated data.


\section{Experimental details}
\subsection{Implementation Details}
\noindent \textbf{Cross-Attention Controlling.} 
Building upon image editing techniques based on diffusion models~\cite{hertz2022prompt}, we find that controlling the cross-attention map can control generation outcomes. In our 2D image generation experiments, modifying viewpoint-specific keywords like \textit{``back''} allows us to transform front-facing images into accurate back-view perspectives without changing the image's structure or subject. Therefore, we propose that controlling cross-attention can reduce viewpoint bias and improve 3D optimization balance. Figure~\ref{fig:sup_1} illustrates the effects of adjusting weights to gradually remove positive features.

We employ the random uniform viewpoint sampling strategy from DreamFusion, with rotation angle ranges defined for front, side, and back views as $[-60^\circ, 60^\circ)$, $[-120^\circ, -60^\circ) \cup [60^\circ, 120^\circ)$, and $[-180^\circ, -120^\circ) \cup [120^\circ, 180^\circ)$, respectively. To emphasize side and back views, we apply weighting factors of $5 \times \text{prompt length}$ and $10 \times \text{prompt length}$, respectively. We modify the \texttt{AttnProcessor2} method in Diffusers to reweight the cross-attention map accordingly.




\noindent \textbf{CLIP Pruning.} 
We attribute the Janus Problem to the long-tail distribution in training data, allowing us to apply methods designed for such distributions. We identify two strategies to address long-tail issues: modifying classifiers and rebalancing sampling. Although classifier guidance~\cite{dhariwal2021diffusion} inspired us, initial experiments using CLIP guidance to generate tail classes~\cite{sehwag2022generating} were unsuccessful due to the generic Open-CLIP~\cite{ilharco_gabriel_2021_5143773,radford2021learning} not being trained on noisy images.

Therefore, we adopt a rebalanced sampling strategy. We treat all pseudo-ground truth outputs from the diffusion model as a potential optimization database, which is imbalanced in front, side, and back views. Unlike DreamControl~\cite{huang2024dreamcontrol}, which rebalances sampling ratios based on computed confidence intervals, we rebalance optimization by pruning incorrect viewpoint images without explicitly calculating confidence intervals.

In our experiments, we used the viewpoint classifications of \textit{``front view,''} \textit{``side view,''} and \textit{``back view,''} converting them into textual embeddings using CLIP. For each iteration, we transformed the pseudo-ground truth \( \bar{x}_0 \) from latent space to pixel space via the VAE. We then embedded the resulting image using CLIP to compute its similarity with the viewpoint embeddings.


\noindent \textbf{Coarse to Fine.} This prompt-based optimization strategy was proposed due to the diffusion model's limited ability to comprehend long prompts.  To address this, we split complex prompts into two components: a simple object description and a descriptive short phrase. During the initial stages, we focus on optimizing the geometric features of the object itself. This process can be regarded as a simplified version of 3D editing techniques.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=1\linewidth]{figs/sup_2.png}
    \vspace{-0.8em}
    \caption{By increasing the weight of the token "back," previously misgenerated images were able to produce accurate back-view features. The left side shows the original generation by SD1.4 for the given prompt, while the right side displays the results after amplifying the weight of ``back."}
    \vspace{-1.0em}
    \label{fig:sup_2}
\end{figure}

\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/sup_3.png}
    \caption{Additional SFCG generation.}
    \vspace{-1.0em}
    \label{fig:sup_3}
\end{figure*}
\subsection{Evaluation Metrics}
\noindent \textbf{Janus Rate.} 
To evaluate geometric consistency, we calculated the occurrence rate of the Janus Problem (JR), defined as the presence of multiple distinct front-view features, such as faces, ears, or noses.
\noindent \textbf{View Dependent CLIP-Score.} 
The CLIP-Score (CS), based on CLIP similarity, measures generation quality by evaluating the similarity between the rendered images of the generated object and the input prompt. However, this metric is not suitable for directly assessing geometric inconsistencies, as front-facing features can significantly boost image-text similarity, even when these features erroneously appear on the object's back.

To address this issue, we designed a view-dependent CLIP-Score. Following the same viewpoint classifications, we append \textit{``* view''} to the original prompt, where * represents \textit{``front,''} \textit{``side,''} or \textit{``back.''} We then render four images of the 3D object from viewpoints at \(0^\circ\), \(90^\circ\), \(180^\circ\), and \(270^\circ\) and calculate their similarities with the modified prompts respectively. The final score is computed as the mean of these similarity scores.

\section{Additional quantitative studies}
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/sup_4.png}
    \caption{Failure Case}
    \vspace{-1.0em}
    \label{fig:sup_4}
\end{figure*}

In this section, we conducted a detailed evaluation of the effectiveness of each component in SFCG. First, we compared the impact of different versions of Stable Diffusion on the Janus Problem. Subsequently, we performed additional ablation studies on the individual components. 

Using DreamFusion~\cite{poole2022dreamfusion} as the baseline, we randomly generated “a DSLR photo of a corgi puppy” five times and calculated the average of the Janus Rate.

\subsection{Comparison of different SD versions}

In the random generation experiment, the baseline of SD1.4~\cite{rombach2022high} has Janus Problem for all generations. The Janus problem of SD2.1 is smaller than that of SD1.4, but still obvious.
SFCG has shown an obvious mitigation effect on the Janus Problem in both versions.

\begin{table}[!htbp]
\centering
\begin{tabular}{|c|c|c|}
\hline
   & SD1.4 & SD2.1 \\ \hline
Dreamfusion & 100\% & 60\% \\ \hline
Dreamfusion+SFCG & 40\% & 20\% \\ \hline
\end{tabular}
\caption{Qualitative comparison of the effects of SFCG on different versions of Stable Diffusion}
\label{tab:example_table}
\end{table}

\subsection{Quantitative ablation comparison}

We conducted experiments by individually adding each of the three components. All three methods demonstrated mitigation effects on the Janus Problem. The experiment was also an average of five randomly generated in DreamFusion.


\begin{table}[!htbp]
\centering
\begin{tabular}{|c|c|c|}
\hline
   & JR \\ \hline
Dreamfusion & 100\%  \\ \hline
+structure feature & 40\%  \\ \hline
+CLIP & 80\%  \\ \hline
% +Coarse to Fine & 60\%  \\ \hline
\end{tabular}
\caption{Qualitative comparison of the effect of different components of SFCG.}
\label{tab:example_table}
\end{table}



\section{More Visualization Results}
Figure~\ref{fig:sup_3} presents additional visual results. The attached video shows the 360-degree comparison with LucidDreamer Baseline.


\section{Failure Case}
Figure~\ref{fig:sup_4} shows some of our failure cases. This can be summarized as follows: the Janus problem on the back is  gone, but there are additional frontal features such as eyes or ears at the transition between the front and the side. We think that the reasons may lie in two aspects. First, side-view images in the training data of diffusion models often contain partial frontal features. Second, when adjusting the weights of cross-attention, this region is typically deprioritized.

